Robots that Learn to Safely Influence via Prediction-Informed Reach-Avoid Dynamic Games

Robots can influence people to accomplish their tasks more efficiently: autonomous cars can inch forward at an intersection to pass through, and tabletop manipulators can go for an object on the table first. However, a robot's ability to influence can also compromise the safety of nearby people if naively executed. In this work, we pose and solve a novel robust reach-avoid dynamic game which enables robots to be maximally influential, but only when a safety backup control exists. On the human side, we model the human's behavior as goal-driven but conditioned on the robot's plan, enabling us to capture influence. On the robot side, we solve the dynamic game in the joint physical and belief space, enabling the robot to reason about how its uncertainty in human behavior will evolve over time. We instantiate our method, called SLIDE (Safely Leveraging Influence in Dynamic Environments), in a high-dimensional (39-D) simulated human-robot collaborative manipulation task solved via offline game-theoretic reinforcement learning. We compare our approach to a robust baseline that treats the human as a worst-case adversary, a safety controller that does not explicitly reason about influence, and an energy-function-based safety shield. We find that SLIDE consistently enables the robot to leverage the influence it has on the human when it is safe to do so, ultimately allowing the robot to be less conservative while still ensuring a high safety rate during task execution.

==> sections/experiments.tex <==

\section{Experimental Setup}
\label{sec:experiments-setup}

\para{Task: Tabletop Object Reaching} We deploy our framework in a scenario where a human and robot arm need to reach their desired objects on the table, but they do not know who is going for what object. 
They must choose objects without colliding into each other. 
We instantiate four objects on the table, two mugs and two bottles (shown in \figref{fig:front_fig}) denoted by $g_i \in \mathcal{G}$ in Cartesian space (i.e. end-effector goals) and via discrete semantic class, $c: \mathcal{G} \rightarrow \mathbb{W}$.
% We assume that the two agents have a fixed set of known objects which are represented by their position in Cartesian space. 
% There are $N$ possible goal states $g_i \in \mathcal{G}$ in Cartesian space (i.e. end-effector goals). 
% These goals each have a corresponding object type, or generally some discrete semantic class, represented by the function $c: \mathcal{G} \rightarrow \mathbb{W}$.
% In the best case, the human and robot will each pick a different object and complete the task quickly. \RP{next sentence is clunky but we need to say this somehow} However, this will not happen without some coordination, so the two agents need to cooperate with the other to properly choose objects---meaning that each of their intended goals may \textit{change depending on the other's actions} while they arbitrate. 


\para{Human-Robot System Dynamics} We model the human and robot as 2-link planar manipulators (i.e. no gravity) and each agent $i\in\{\human,\robot\}$'s dynamics are:
\begin{equation}
    M_i(q_i)\Ddot{q}_i + C_i(q_i,\dot{q}_i)\dot{q}_i = B_iu_i,
\end{equation}
where the state $q_i\in \qSpace_i$ consists of the joint angles, $M_i$ is the inertia matrix, $C_i$ captures Coriolis forces, and $B_i$ represents how the control input affects the system. 
The agents' actions $\ctrl_i\in\ctrlSet_i$ are the joint torques bounded by a box constraint: $\ctrlSet_i:=\{\ctrl \mid \ctrl_i^{min} \leq \ctrl \leq \ctrl_i^{max}\}$. 
We model the robot as having larger control authority than the human.
% to ensure there is a solution to the reach-avoid problem. 
%This is a less strict assumption than assuming that humans are quasi-static obstacles, as assumed in previous work \RP{cite}.
The configuration space states $q_i$ are transformed by an observation map $\mathcal{O}_i :\qSpace_i \rightarrow \mathbb{R}^{n_i}$ where $n_i$ is the dimensionality of the observation for agent $i$. 
The physical state input to the model is the concatenation of observations of both agents: $\stateSpace := \mathcal{O}_\robot(\qSpace_\robot) \times \mathcal{O}_\human(\qSpace_\human)$. 
% In this work, the observation map transforms joint angles to their sine and cosine.

\para{Multi-Arm Interaction Data Generation} 
To create our conditional behavior prediction model, we need a dataset of multi-agent interactions to learn from. 
Unlike in autonomous driving, where many large, diverse, multi-agent datasets already exist \cite{ettinger2021large, caesar2020nuscenes, chang2019argoverse}, these types of large datasets are underrepresented in collaborative manipulation. 
We thus choose to create our own synthetic dataset of multi-agent interactions so that we can control how the other agent is influenced can cleanly analyze the effect of our influence-aware safe control policy.
% We start by assuming both agents have a shared set of $N$ possible goal states $\theta_i \in \Theta$ in Cartesian space (i.e. end-effector goals). These goals each have a corresponding object type, or generally some discrete semantic class, represented by the function $c: \Theta \rightarrow \mathbb{W}$. 
Our simulated human always tries to choose an object with a different type than the robot. We simulate this by having the human keep their own belief over the goal that robot is currently choosing, $b_\human^t(g) \propto P(u_\robot^t \mid q_\robot^t, g) b_\human^{t-1}(g)$, which gets updated online via Bayes' Rule. 
% given the robot's current state and action $(q_\robot^t, u_\robot^t)$.
% This means that the human only changes their goal if the robot's most likely goal has both probability $\geq 0.5$ and has the same semantic class as the human's goal. 
The human changes their goal to be the least likely robot goal based on $b_\human^t$ if the robot's most likely goal both has probability $> 0.3$ and has the same semantic class as the human's goal.
The dataset is generated by randomly sampling initial goals for the two agents and rolling out for fixed horizon of 15 seconds.  

\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{figs/traj_rollout_merge.pdf}
    \caption{\textbf{Closed-Loop Simulations.} (left) \ours and \robust policies starting from the same initial condition. SLIDE confidently understands that the human will be influenced to move out of its way as it chooses the blue bottle and reaches the fastest (the human changes its mind from the blue bottle to the yellow mug at $t=1.2s$). 
    % Marginal-RA waits until the human is out of its way and chooses the bottom mug. 
    Robust-RA stays cautious even as the human is moving towards a different goal and finishes last. (right) When interacting with a non-influenceable human, \ours tries to influence them to choose the red bottle, but eventually backs off and chooses a safe goal instead (the blue bottle).}
    \label{fig:traj-rollout}
\end{figure*}

% The human changes its current goal $g_\human^t$ based on $b_\human^t$ using the following rule:
% \begin{equation}
%     \theta_\human^{t+1} = 
%     \begin{cases}
%         g_\human^t, & \text{if } \argmax{g\in\mathcal{G}} b_\human^t(g) < 0.5 \\
%         \argmin{g \in \mathcal{G}} b_\human^t(g), & \text{if } c\left(\argmax{g\in\mathcal{G}} b_\human^t(g)\right)= c(g_\human^t) \\
%         g_\human^t, & \text{otherwise.}
%     \end{cases}
% \end{equation}



% \abnote{Describe how we need a dataset of multiple agents interacting to train our model.  We generate our own dataset for two reasons: (1) we can control exactly how the other agent is influenced to focus all of our questions / analysis on just the influence-aware safety filter, (2) unlike autonomous driving where there is plentiful data, these types of datasets are still very underrepresented in collaborative manipulation. However, future work should relax this. Then describe the process for how you simulate this data}


\para{Methods} We compare two human prediction models: marginal and conditional (CBP). We also compare our method, \ours, with four other robot policies: \nosafety (computed torque control), the Safe Set Algorithm (\ssa) \cite{liu2014control}, Robust reach-avoid (\robust) \cite{hsu2023isaacs}, and Marginal reach-avoid (\marginal) \cite{hu2023deception}. We use a naive version of SSA to understand the effect of adding simple safe control. The robust policy solves the same reachability problem but without including a prediction model, and the marginal policy has the same structure as SLIDE but its prediction model is not conditioned on the robot's future plan. 

% \abnote{In our experiments, four robot policies: no-safety, static-obs-CBF \todo{cite}, robust-RA \todo{cite}, marginal-RA \todo{cite}, and CBP-RA. And within our prediction-informed methods, we compare two human prediction models: Marginal, CBP.}

\para{Metrics} For trajectory prediction models, we measure the average displacement error (ADE), final displacement error (FDE), and size of the inferred control bound $|\ctrlSetH|$. For closed-loop simulations of the agents, we measure: 1) collision rate (safety) 2) task completion rate (liveness) and 3) completion time (average trajectory length). 
% \abnote{For forecasting, we measure ADE/FDE. For safety value function learning, we measure FP/FN..... For closed-loop simulations of each robot policy, we measure: (1) collision rate (safety), (2) goals reached (liveness), (3) safety override rate, (4) average trajectory length (task completion speed).}

\para{Training: Prediction Models for Manipulation} The prediction models are both 3-layer MLPs\footnote{We found this simple architecture to be sufficient for our task, but our method is agnostic to the complexity of the model.} with hidden sizes of 256 neurons and output the parameters of a Gaussian Mixture Model (GMM) to predict the human's actions for the next 1 second. Both models' input consists of a 1-second history of both agents' end effector positions, the goal positions $\Theta$, and the goals' semantic classes $c(\theta_i)$ as a flattened vector. The CBP model additionally takes in a 2-second future plan of the robot's end effector position. The models are trained with the sum of two loss function terms (similar to \cite{tolstaya2021identifying}): 1) negative log-likelihood and 2) MSE of most-likely GMM mode. 

% \abnote{Describe how you train, loss function, hyperparameters, etc. Describe the difference in the CBP vs. the marginal predictor.}

\para{Training: Safety Value Function} The actor and safety critic networks are 4-layer MLPs with a hidden size of 256 and the actor outputs a Guassian distribution for the action of the robot. The input to the networks consists of the 24D observed state (plus 15D extended belief state for marginal and SLIDE methods). The belief state consists of the mode means and mixture weights of the trajectory predictor's GMM output.
The policies are trained using one NVIDIA GeForce RTX 4090 GPU and the RL environment is run on 16 parallel threads on an AMD Ryzen Threadripper 7960X CPU. The wall-clock time for training the robust policy is approximately 5 hours, the marginal policy is approximately 28 hours, and SLIDE is 61 hours. This includes time for pretraining the ego and adversary agents, following the training scheme laid out by \cite{hsu2023isaacs}. 

% \abnote{Describe the training process, hyperparameters, compute you use, how long it takes, etc. Describe how the main change between these for robust vs. marginal vs. CBP is how we restrict the action space of the opponent during training. }

\section{Experimental Results}
\label{sec:experiments-results}
% thinking out loud:
% \begin{itemize}
%     \item what do we want to answer? the main question is basically just this: do where can we get improvements over using a marginal predictor to construct the belief space? this should mean we need to show non-inferiority on average, and improvement in important highly interactive scenarios
%     \item this also means we want to look at situations where either 1) marginal predictor itself is insufficient or 2) the resulting safe controller from the marginal predictor is more conservative than it needs to be 
%     \item one big question then becomes: what happens when the \textit{influence-aware} model is overly confident? do we recover well/continue to be safe when there is misaligned influence behavior (model assumes human will change but they actually don't)? if we do get robustness to this, then it's interesting as a potential response/mitigation to the one Tomizuka paper's criticism of CBP models 
%     \item above basically points to an approach that does something confidence-aware, essentially thomas' paper. fundamentally, what's different about this work vs that one? the difference on a basic level is that this works on higher dimensional systems. more fundamentally, I think the difference is about including the belief inside the observation space instead of doing a belief-based averaging
%     \item we want to know how well the model is able to preemptively predict when the human agent will be influenced (basically show that the influence-aware predictor gets to choose a plan that the marginal and robust versions do not, since they don't know that the human will change goals in response). maybe this means we want to show the robot ``bullying'' the human in terms of goal choice
% \end{itemize}\textbf{}

%% we won't report this for now, since ISAACS RA value function tends to be overly conservative relative to the trained policy
% \subsection{On the quality of approximating RA safety}
% \abnote{We report the statistics about the quality of learning each of our methods. Takeaway: its reasonable, and similar to the original statistics from the reach-avoid RL paper.}

\subsection{Influence-Aware vs. Influence-Unaware Safety}

We first study the closed-loop performance of \ours's controller, which safely exploits influence, compared to alternative safe controllers described in \sref{sec:experiments-setup}. 
% When evaluating the trained policies, we simulate the human by having them play according to the same data distribution as described in \sref{sec:experiments}. We later ablate this to study the sensitivity of our approach to out-of-distribution human partners.

% \abnote{Assume that the simulated human is playing according to the data distribution from section above. We will later ablate this to study the sensitivity of our approach. }

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/time_hist_single.pdf}
    \caption{\textbf{Closed-loop Completion Times.} Histogram of completion times for all methods interacting with the influenceable human model. 
    \ours has the highest frequency of short trajectories, while \ssa and \robust have the highest incidence of timing out.}
    \label{fig:time_hist}
    \vspace{-0.5em}
\end{figure}

\begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|c c c c}
        \toprule
         & \multicolumn{1}{c}{Collision rate} & \multicolumn{1}{c}{Completion rate} & \multicolumn{1}{c}{Completion Time (s)} \\
        \midrule
        \nosafety & $28.5\%$ & $71.5\%$ & $3.5\pm 1.8$ \\
        \ssa & $19.1\%$ & $52.3\%$ & $8.9 \pm 4.7$ \\
        \robust & $1.4\%$ & $97.0\%$ & $2.6 \pm 2.1$ \\
        \marginal & $1.5\%$ & $98.0\%$ & $2.5\pm 1.3$ & \\
        \ours (ours) & $1.9\%$ & $98.1\%$ & $1.9\pm 0.8$ \\
        \bottomrule
    \end{tabular}
    }
    \caption{\textbf{Closed-loop Results. } Failure rate, completion rate and completion time for all methods over 1,000 randomized trials. The task is incomplete if the robot does not reach any goal within 15 seconds. \ours is able to reach its goal most often and in the shortest time without becoming significantly less safe.}
    \label{tab:policy_eval}
    \vspace{-0.1in}
\end{table}

\para{Results: Quantitative}
\tabref{tab:policy_eval} shows all methods' performance. As expected, \robust has the smallest collision rate and all safe controllers have a lower collision rate than \nosafety.
However, what \robust and \marginal gain in safety, they lose in completion rate and time. In contrast, \ours has the highest completion (liveness) rate while having a comparable collision rate to the robust and marginal baselines. 
% not significantly increasing the collision rate relative to the robust and marginal reach-avoid policies. 
Moreover, \ours allows the robot to reach goals significantly faster: e.g., $24\%$ faster than \marginal. 
We further plot the histogram of completion times  in \figref{fig:time_hist}. 
We see that \ours almost never times out, while other methods do. 
We note that \ssa collides and times out the most out of the safe controllers. 
The reason for this is because the safety index for \ssa was hand-tuned (as proposed in \cite{liu2014control}), so it does not always respect the system's control limits. If we used some additional safety index synthesis techniques \cite{zhao2023safety} to properly account for the control bounds, the performance would likely approach that of \robust, though without the goal-reaching policy built-in.
% We hypothesize this is because \ssa is computed by calculating the time derivatives of the distance between the closest points on the two arms at each timestep, so when these points make a discrete jump (i.e. the closest point changes from one link to another), the controller is unable to preempt this and results in collisions. Additionally, similar to many control-barrier-function-style methods, accounting for 
% % synthesizing a valid safety index in the presence of 
% control constraints is nontrivial and requires careful manual tuning. 
% % ---the nominal safety index we use often requires safe controls that are outside the allowable control bounds for the robot. 

\para{Results: Qualitative} We visualize \ours and \robust's closed-loop trajectories in \figref{fig:traj-rollout}. 
% To understand why SLIDE results in faster trajectories, we can look at . 
\robust initially keeps the robot arm far away from all goals, waiting for the human to move out of the way before reaching for a mug.
% as the human agent is moving towards its own goal. 
% The robust and marginal controllers both wait for the human to move out of the way before reaching for the goal closest to them, with marginal able to reach slightly faster.
In contrast, \ours immediately recognizes that it can influence the human's target object (bottom, \figref{fig:traj-rollout}). It switches to reach the bottle, ensuring the human picks a cup, stays out of its way, and enables the robot to complete the task faster. 

\subsection{Ablation: When Does Modeling Influence Matter?}
Next, we study when it matters that we use influence-aware human models for safe control. 
We ablate if the robot uses a \textit{conditional} or \textit{marginal} prediction model (i.e. no conditioning on robot's future plan).
We compare both the performance of the predictors and their effect on the learned reach-avoid policies. 

% \abnote{here we ask the question, when does it matter that I'm injecting this CBP into my safety filter? we will still assume that the simulated human is playing according to the data distribution, but we now explicitly compare marginal-RA and CBP-RA.}

\begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|c|| c c c}
        \toprule
         & \multicolumn{1}{c||}{All Data (14,000)} & \multicolumn{1}{c}{Interactive Data (2,457)} & \multicolumn{1}{c}{Non-Interactive Data (11,543)} \\
        \midrule
        % \textbf{Marginal} & $0.002\pm0.004$ ($0.12 \pm 0.24$) & $0.007 \pm 0.006$ ($0.40 \pm 0.30$) & $0.001 \pm 0.002$ ($0.07 \pm 0.18$) \\
        % \textbf{CBP} & $0.001\pm 0.003$ ($0.09 \pm 0.20$) & $0.007\pm 0.002$ ($0.30 \pm 0.29)$ & $0.0007 \pm 0.002$ ($0.04 \pm 0.13$) \\
        \textbf{Marginal} & $0.002$ ($0.12$) & $0.007$ ($0.40$) & $0.001$ ($0.07$) \\
        \textbf{CBP} & $0.001$ ($\textbf{0.09}$) & $0.007$ ($\textbf{0.30}$) & $0.0007$ ($\textbf{0.04}$) \\
        \bottomrule
    \end{tabular}
    }
    % \vspace{0.1em}
    \caption{\textbf{Open-Loop Prediction Error.} Average (ADE) and Final Displacement Error (FDE) of marginal and CBP predictors.}
    \label{tab:cbp-v-marg}
\end{table}

\begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|c|| c c c}
        \toprule
         & \multicolumn{1}{c||}{All Data (14,000)} & \multicolumn{1}{c}{Interactive Data (2,457)} & \multicolumn{1}{c}{Non-Interactive Data (11,543)} \\
        \midrule
        \textbf{Marginal} & [12.3, 12.7] & [13.8, 13.6] & [11.9, 12.5] \\
        \textbf{CBP} & [7.8, 8.3] & [12.7, 12.9] & [6.7, 7.3] \\
        \bottomrule
    \end{tabular}
    }
    % \vspace{0.1em}
    \caption{\textbf{Inferred $\ctrlSet_\human$ Size.} Average inferred control bound size from \marginal ($|\ctrlSetH|$) and \ours ($|\ctrlSetH(\aRtraj)|$). Entries shown per ctrl. dimension and the max. dyn. feasible range is 20.}
    \vspace{-1.5em}
    \label{tab:cbp-v-marg-bounds}
\end{table}

\para{Approach} In these experiments, the human agent acts according to the data distribution in \sref{sec:experiments-setup}. 
We evaluate the predictors on a dataset  $\mathcal{D}$ of 100 held-out trajectories, each 15 seconds long, resulting in 14,000 data points\footnote{We discount predictions in the last 1 second of each trajectory since this is length of the prediction horizon.}.

\para{Open-Loop Results: Quantitative \& Qualitative} 
% The ADE is measured as the average L2 distance of the predicted end-effector position from the \textit{first timestep} of the prediction horizon vs the true end-effector position. 
% The FDE is measured as the L2 distance between the end-effector position predicted for the \textit{final timestep} of the prediction horizon vs the true end effector position at the corresponding timestep. 
\tabref{tab:cbp-v-marg} shows ADE and FDE results. Averaged across the held-out dataset, ADE looks very similar for both marginal and CBP, with CBP performing better on FDE (left, \tabref{tab:cbp-v-marg}). 
However, only a \textit{subset} of all trajectories in this held-out dataset exhibit highly interactive scenarios. 
% In this work, we're also particularly interested in interactive scenarios. 
% However, these are are long-tail events \cite{tolstaya2021identifying}, 
Thus, we further decompose dataset $\mathcal{D} = \mathcal{D}_I \cup \mathcal{D}_{\neg I}$ into data points where influence is happening $\mathcal{D}_I$ (2,457 data points) and those where it is not $\mathcal{D}_{\neg I}$ (11,543 data points). 
This is done by tracking the timesteps where the human's goal changes: if it does, then this and directly adjacent timesteps are added to $\mathcal{D}_{I}$. 
For data in $\mathcal{D}_{I}$, the CBP model has a significantly lower FDE compared to the marginal trajectory predictor (center column, \tabref{tab:cbp-v-marg}), indicating that the CBP matters to predict long-term behavior in highly interactive scenarios.
\figref{fig:cbp_predictions} shows the CBP model that \ours uses as a function of the robot's plan. 
Each robot plan results in distinct human predictions. This capability (not present in a marginal prediction model) gives the \ours policy the freedom to learn which goals to move towards to best influence the human to move out of its way.
% a stark improvement over the marginal predictor on these scenarios, despite also degrading in performance. 
We further study the implications of each model on the inferred control bounds, $\ctrlSetH$, that we use during reach-avoid computations (\sref{sec:method}). 
This will directly tell us how the prediction model will affect the policy training loop, since this determines the set of allowable actions for the adversary agent. 
% Although we see that the CBP model does better on the task of prediction, we're ultimately interested in understanding how this will affect the downstream closed-loop performance of the trained reach-avoid policies. 
% To investigate this, we measure the average size of the inferred control bound (\sref{sec:method}) on this dataset. 
% the error rates look very similar, with the CBP model doing slightly better. 
% However, we know that highly interactive scenarios are long-tail events \cite{tolstaya2021identifying}, so we decompose the datasets into data points where influence is happening $\mathcal{D}_I$ (2457 data points) and those where it is not $\mathcal{D}_{\neg I}$ (11,543 data points). This is done by tracking the timesteps where the human's goal changes---if it does, then this and directly adjacent timesteps are added to $\mathcal{D}_{I}$. We now uncover a stark difference in the FDE when considering only $\mathcal{D}_I$. While both predictors degrade, the CBP model performs better than the marginal predictor. 
% To understand how this difference will affect the downstream policies, we measure the average size of the inferred control bound (\sref{sec:method}) on this dataset. 
In \tabref{tab:cbp-v-marg-bounds} we show the  size of the inferred control bounds. The CBP action bounds enlarge at interactive states, but do not expand as much as the marginal predictor's bounds.
On the full dataset, the CBP model results in a smaller control bound on average. 
This implies that \ours's downstream policy (which uses the CBP) will be able to exploit the human's influence and thus choose less conservative actions. 
% while playing against the restricted opponent agent during training. 

\para{Closed-Loop Results: Quantitative \& Qualitative} Finally, we study the closed-loop safety and liveness performance of of the \ours policy and the \marginal policy. 
In \tabref{tab:policy_eval}, we see that both methods have a similar task completion rate (\ours is 98.1\% while \marginal is 98.0\%). 
However, the main difference comes in their completion \textit{time}: \ours completes the task in $1.9s$ compared to \marginal at $2.5s$. This implies that our SLIDE policy exploits the influence it has on the human to maximize task completion efficiency. 
Qualitatively, we see that \ours chooses the top bottle (top right, \figref{fig:front_fig}) to influence the human into picking to the bottom mug, making the two agents stay out of each others' way. 
In contrast, the \marginal policy chooses the goal closest to itself, but then must wait for the human to move out of the way before reaching the goal. 

% In \tabref{tab:policy_eval}, we see that SLIDE has a completion rate of 99.3\%, while Marginal-RA has a completion rate of 97.7\%, while both have the same collision rate of $0.6\%$. This means that SLIDE is able to reach goals more often than the Marginal-RA policy without incurring any additional safety violations. We also see that SLIDE has a lower average completion time at $2.2s$ compared to Marginal-RA's $2.4s$, meaning that the SLIDE policy understands when it is safe to move faster towards its goal.

% \abnote{closed-loop results: \textbf{M1:} measure the \% states that are now safe \& live in the CBP-RA that weren't in the marginal-RA. The bigger, the better. Means that it "matters"} \todo{run statistics like these--since this is no longer a safety shield, we can only directly measure through rollouts, though not sure how this is different from \tabref{tab:policy_eval} }

% \abnote{\textbf{M2:} We have this dataset of 1,000 initial conditions and their rollouts of the human behavior. If you look at the average across 1,000 initial conditions, it at first appears as though the two models perform similarly. But we know that these influence-aware scenarios are long-tail events, so we decompose the dataset into scenarios where there is influence $\mathcal{D}_I$ (100 scenarios) and where there isn't $\mathcal{D}_{\not I}$ (900). The way we do this is by tracking when the simulated human changes their target goal---if they did, we mark this interaction as one where influence happened. Update \ref{tab:cbp-v-marg} training and closed-loop results}

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\columnwidth]{figs/cbp_predictions.pdf}
    \caption{\textbf{Conditional Behavior Predictions.} Most-likely mode of \ours CBP model given different future robot plans. Each robot plan has a corresponding human prediction in the same color. The prediction is highly dependent on the robot's plan and captures the idea that the human will change goals to a different semantic class.}
    \label{fig:cbp_predictions}
    \vspace{-1em}
\end{figure}

% \para{Open \& Closed-Loop Results: Qualitative} 
% \abnote{remove below?}
% \figref{fig:traj-rollout} shows the the main factor in allowing SLIDE to reach its goal more efficiently is its choice of goal. Since it understands the long-term influence it can have on the human partner, it chooses the top bottle to influence the human into picking to the bottom mug, making the two agents stay out of each others' way. The Marginal and Robust policies instead choose the goal closest to themselves, but this means they both need to wait for the human to move out of the way before actually reaching this goal. 

% In \figref{fig:traj-rollout}, we can see two important factors that result in SLIDE reaching its goals more efficiently than Marginal-RA. First, the SLIDE controller moves much closer to the human early on, since its prediction model is more confident. Next, it actively chooses a trajectory that influences the human's goal to be different from the robot's at all points in the trajectory. The Marginal-RA policy causes the human to infer its goal incorrecrtly for a few timesteps, resulting in the two agents reaching for a same goal, meaning it needs to be more cautious on its way towards its own goal.
% \abnote{Show a candidate scenario in-line that shows this gap}
% discuss how the resulting safety filter acts differently than one using a marginal predictor (qualitatively: figure with snapshots of a rollout) and quantitatively (higher safety+liveness rate on particular initial conditions, or shorter trajectories on those conditions)
% \abnote{The reason we see this gap is precisely because the influence-aware reachability controller choose goals that influence the human's goal?} - check to see if/when the human's goal changes as a result of the robot's controller

\subsection{How Robust is SLIDE to Out-of-Distribution Humans?}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{figs/no_influence.pdf}
%     \caption{Shows an interaction between the SLIDE controller and a stubborn (non-influenceable) human model. The modes of the GMM output by the CBP prediction model are visualized as dots from the human's end effector. %At first, SLIDE tries to influence the human to choose a far away goal. Once it cannot change the human's goal, it eventually backs off and chooses another safe goal. We can see that even though the prediction model thinks the human will most likely move, one of the modes covers the possibility of the human not moving, so the SLIDE controller can react to this outcome.
%     }
%     \label{fig:no_influence}
%     \vspace{-0.25in}
% \end{figure}

Finally, we study how robust the \ours policy is 
% one concern with injecting a prediction model into 
% is that the prediction model may degrade 
when interacting with human behavior that is out-of-distribution (OOD) from the conditional behavior prediction model. We measure the same closed-loop metrics described in \sref{sec:experiments-setup}. 

\para{Approach}
We ablate the deployment-time human model (right, \figref{fig:system_diagram}) to be OOD relative to the prediction model training data.  
Specifically, we change the human to be \textbf{non-influenceable} (also referred to as \textit{stubborn}) and \textbf{adversarial} (where the human always chooses the goal it thinks the robot is likely moving towards\footnote{Note that this is different from the optimal disturbance policy $\pi_\human^\dagger$ trained in simulated gameplay.}). 
% , since these may result in the CBP model being overconfident that the human will move out of the robot's way.

% \begin{table}[ht]
%     \centering
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l|c c c c}
%         \toprule
%          & \multicolumn{1}{c}{Collision rate} & \multicolumn{1}{c}{Completion rate} & \multicolumn{1}{c}{Completion Time (s)} \\
%         \midrule
%         \textbf{No-Safety} & $22.8\%$ & $77.2\%$ & $3.6 \pm 1.8$ \\
%         \textbf{SSA} & $10.4\%$ & $40.7\%$ & $10.5\pm 5.0$ \\
%         \textbf{Robust-RA} & $1.1\%$ & $93.9\%$ & $3.0\pm 3.0$ \\
%         \textbf{Marginal-RA} & $1.2\%$ & $98.0\%$ & $2.5\pm 1.5$ & \\
%         \textbf{SLIDE (ours)} & $1.8\%$ & $98.1\%$ & $2.0 \pm 0.9$ \\
%         \bottomrule
%     \end{tabular}
%     }
%     % \vspace{0.1em}
%     \caption{Comparison of methods when interacting with a \textbf{stubborn (non-influenceable)} human (OOD from trained model) over 1000 randomized trials. SLIDE does result in a slightly higher collision rate, but is still better than the no-safety baseline and reaches its goal faster than all baselines.}
%     \label{tab:policy_eval_stubborn}
% \end{table}

% \begin{table}[ht]
%     \centering
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l|c c c c}
%         \toprule
%          & \multicolumn{1}{c}{Collision rate} & \multicolumn{1}{c}{Completion rate} & \multicolumn{1}{c}{Completion Time (s)} \\
%         \midrule
%         \textbf{No-Safety} & $22.8\%$ & $77.2\%$ & $3.6 \pm 1.8$ \\
%         \textbf{SSA} & $15.0\%$ & $37.7\%$ & $10.3\pm 5.0$ \\
%         \textbf{Robust-RA} & $1.5\%$ & $98.3\%$ & $2.5\pm 1.6$ \\
%         \textbf{Marginal-RA} & $2.2\%$ & $97.0\%$ & $2.6\pm 1.5$ & \\
%         \textbf{SLIDE (ours)} & $3.8\%$ & $96.2\%$ & $1.9 \pm 0.7$ \\
%         \bottomrule
%     \end{tabular}
%     }
%     % \vspace{0.1em}
%     \caption{Comparison of methods when interacting with an \textbf{adversarial goal-selecting} human (OOD from trained model) over 1000 randomized trials. The human always chooses the goal it thinks the robot is moving towards. SLIDE and marginal policies result in higher collision rates compared to the robust policy.}
%     \label{tab:policy_eval_adv}
% \end{table}

\begin{table}[t!]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|c c c c}
        \toprule
         & \multicolumn{1}{c}{Collision rate} & \multicolumn{1}{c}{Completion rate} & \multicolumn{1}{c}{Completion Time (s)} \\
        \midrule
        \textbf{Influenceable Human} & $1.9\%$ & $98.1\%$ & $1.9\pm 0.8$ \\
        \textbf{Stubborn Human (OOD)} & $1.8\%$ & $98.1\%$ & $2.0\pm 0.9$ \\
        \textbf{Adversarial Human (OOD)} & $3.8\%$ & $96.2\%$ & $1.9\pm 0.7$ \\
        \bottomrule
    \end{tabular}
    }
    % \vspace{0.1em}
    \caption{\textbf{Closed-Loop OOD Human Results.} \ours interacts with in-distribution and out-of-distribution (OOD) humans over 1,000 randomized trials. 
    Stubborn human never changes their goal. Adversarial human always chooses the goal it thinks the robot is moving towards. SLIDE is relatively robust to the stubborn human, but starts to degrade against the adversarial human.}
    \label{tab:policy_eval_ood}
    \vspace{-1em}
\end{table}

\para{Results: Quantitative \& Qualitative} 
Results are shown in \tabref{tab:policy_eval_ood}
for 1,000 random initial conditions. 
We see that when interacting with a stubborn human, \ours generally performs similarly to the in-distribution human model. %Qualitatively, we find that the Robust controller tends not to move when the human has already reached a goal and is stationary; this is likely an artifact of the adversarial RL training loop. 
We hypothesize this is precisely because of the \textit{inference hypothesis} from \sref{sec:method}: instead of blindly trusting the output, we allow the simulated opponent agent to take any $\delta-$likely action from $\epsilon-$likely modes. 
This means as long as the modes of the prediction model have some coverage of the agent's true behavior, the learned policy will still be robust to it. 
We can see an example of this in the right side of \figref{fig:traj-rollout}. 
At first, \ours tries to influence the human to switch to the red bottle goal. 
% , and we can see that the prediction model's most likely future for the human is to move away. 
After a few timesteps, however, \ours backs off and chooses a different (safe) goal (the blue bottle) to complete the task.
When interacting with the \textbf{adversarial human} that always chooses the goal it thinks the robot is moving towards, we can see that \ours starts to collide more often (bottom row, \tabref{tab:policy_eval_ood}). 
This makes sense since the human sometimes takes actions that are in direct opposition to the predictor's training data, which our inference hypothesis is unable to account for. 
% so even unlikely modes may not have covered this kind of data. 
However, it is a promising sign that there is not a catastrophic degradation in the collision rate.
Future work should investigate, for example, the use of a \textit{hybrid} approach which switches between the \robust controller and \ours depending on the prediction quality observed during deployment. 
% This result points us in the direction of wanting to allow a prediction-reliant method like SLIDE to fall back on a robust policy when the true observed human data is far out of distribution. 
% A confidence-aware approach was taken in \cite{tian2022safety}, but it is unclear how this approach can scale to RL-based safety controllers like we use in this paper. 

%\RP{you could probably do this detection with conformal prediction; instead of smoothly varying from CBP to robust, just have a switching threshold}

% Robust-RA, Marginal-RA and SLIDE methods all have worse completion rates when interacting with a non-influencable human---since the human never gets out of the robot's way, the methods will time out more often. The Robust-RA method keeps the same collision rate as before, but the Marginal-RA and SLIDE methods both collide more often than Robust-RA. This also makes sense, since the trajectory predictors will more often be wrong about this OOD human policy.

% However, we do not see a catastrophic degradation in the collision rate when dealing with this non-influencable human mode. We believe this the reason is because the robot does not blindly trust the prediction model during training, but instead considers staying robust any $\delta-$likely action within all $\epsilon-$likely mode. Even if the human model is OOD from the training data, as long as at least one (potentially unlikely) mode of the prediction model covers their true behavior, the robot is still able to stay safe around them.
% \RP{plot a scenario where SLIDE collides but robust doesn't?}

% 6. concern: what if the model is \textit{over}confident? does this result in a huge drop in safety (or performance)?
% - this means we need to test against a human that doesn't strictly match the training data distribution of the CBP model. This could be something like changing the likelihood function of bayesian inference, or something simple like testing against a non-influenceable human
% \abnote{ideal takeaway is that the robustness inherent in the RA formulation helps us with these scenarios when just blindly trusting the prediction model on its own may not.}

% \abnote{DREAM eval: compare our CBP-RA to a robot that just does open-loop predictions and open-loop plan at some fixed replanning step. }
